Low Influence, Utility, and Independence in Differential Privacy: A Curious Case of $3 \choose 2$

We study the relationship between randomized low influence functions and differentially private mechanisms. Our main aim is to formally determine whether differentially private mechanisms are low influence and whether low influence randomized functions can be differentially private. We show that differential privacy does not necessarily imply low influence in a formal sense. However, low influence implies approximate differential privacy. These results hold for both independent and non-independent randomized mechanisms, where an important instance of the former is the widely-used additive noise techniques in the differential privacy literature. Our study also reveals the interesting dynamics between utility, low influence, and independence of a differentially private mechanism. As the name of this paper suggests, we show that any two such features are simultaneously possible. However, in order to have a differentially private mechanism that has both utility and low influence, even under a very mild utility condition, one has to employ non-independent mechanisms.

==> tikz/Old/old_delta_dp_3D.tex <==
\begin{tikzpicture}


\begin{axis}[width=6cm, height=6cm,stack plots=y,thick,smooth,no markers,xmin=0,xmax=1,ymin=0,ymax=1,zmin=0,zmax=1,xlabel={$x$},
  ylabel={$y$},zlabel={$z$},xtick={0,0.5,1},ytick={0.5,1},ztick={0.5,1},view={60}{30}]
  

\draw[color=black] (0,0,10) -- (50,0,10);
\draw[color=black] (0,0,20) -- (50,0,20);
\draw[color=black] (0,0,30) -- (50,0,30);
\draw[color=black] (0,0,40) -- (50,0,40);
\draw[color=black] (0,0,50) -- (50,0,50);
\draw[color=black] (0,0,60) -- (50,0,60);
\draw[color=black] (0,0,70) -- (50,0,70);
\draw[color=black] (0,0,80) -- (50,0,80);
\draw[color=black] (0,0,90) -- (50,0,90);
\draw[color=black] (0,0,100) -- (50,0,100);

\draw[color=black] (10,0,0) -- (10,0,100);
\draw[color=black] (20,0,0) -- (20,0,100);
\draw[color=black] (30,0,0) -- (30,0,100);
\draw[color=black] (40,0,0) -- (40,0,100);
\draw[color=black] (50,0,0) -- (50,0,100);

\draw[color=black] (50,0,0) -- (100,50,0);
\draw[color=black] (50,0,10) -- (100,50,10);
\draw[color=black] (50,0,20) -- (100,50,20);
\draw[color=black] (50,0,30) -- (100,50,30);
\draw[color=black] (50,0,40) -- (100,50,40);
\draw[color=black] (50,0,50) -- (100,50,50);
\draw[color=black] (50,0,60) -- (100,50,60);
\draw[color=black] (50,0,70) -- (100,50,70);
\draw[color=black] (50,0,80) -- (100,50,80);
\draw[color=black] (50,0,90) -- (100,50,90);
\draw[color=black] (50,0,100) -- (100,50,100);



\draw[color=black] (100,50,10) -- (100,100,10);
\draw[color=black] (100,50,20) -- (100,100,20);
\draw[color=black] (100,50,30) -- (100,100,30);
\draw[color=black] (100,50,40) -- (100,100,40);
\draw[color=black] (100,50,50) -- (100,100,50);
\draw[color=black] (100,50,60) -- (100,100,60);
\draw[color=black] (100,50,70) -- (100,100,70);
\draw[color=black] (100,50,80) -- (100,100,80);
\draw[color=black] (100,50,90) -- (100,100,90);
\draw[color=black] (100,50,100) -- (100,100,100);


\draw[color=black] (100,50,0) -- (100,50,100);
\draw[color=black] (100,60,0) -- (100,60,100);
\draw[color=black] (100,70,0) -- (100,70,100);
\draw[color=black] (100,80,0) -- (100,80,100);
\draw[color=black] (100,90,0) -- (100,90,100);


\draw[color=black] (0,10,100)  -- (60,10,100);
\draw[color=black] (0,20,100) -- (70,20,100);
\draw[color=black] (0,30,100) -- (80,30,100);
\draw[color=black] (0,40,100) -- (90,40,100);
\draw[color=black] (0,50,100) -- (100,50,100);

\draw[color=black] (60,10,100) -- (60,10,0);
\draw[color=black] (70,20,100) -- (70,20,0);
\draw[color=black] (80,30,100) -- (80,30,0);
\draw[color=black] (90,40,100) -- (90,40,0);
\draw[color=black] (100,50,100) -- (100,50,0);


\draw[color=black] (0,50,100) -- (100,50,100);
\draw[color=black] (10,60,100) -- (100,60,100);
\draw[color=black] (20,70,100) -- (100,70,100);
\draw[color=black] (30,80,100) -- (100,80,100);
\draw[color=black] (40,90,100) -- (100,90,100);

\draw[color=black] (0,50,100) -- (50,100,100);
\draw[color=black] (0,0,100) -- (0,50,100);
\draw[color=black] (0,0,0) -- (0,0,100);
\draw[color=black] (0,0,0) -- (50,0,0);
\draw[color=black] (100,50,0) -- (100,100,0);
\draw[color=black] (100,100,0) -- (100,100,100);
\draw[color=black] (100,100,100) -- (50,100,100);

\draw[color=black] (60,10,100) -- (60,100,100);
\draw[color=black] (70,20,100) -- (70,100,100);
\draw[color=black] (80,30,100) -- (80,100,100);
\draw[color=black] (90,40,100) -- (90,100,100);


\draw[color=black] (10,0,100) -- (10,60,100);
\draw[color=black] (20,0,100) -- (20,70,100);
\draw[color=black] (30,0,100) -- (30,80,100);
\draw[color=black] (40,0,100) -- (40,90,100);
\draw[color=black] (50,0,100) -- (50,100,100);



\filldraw[color=blue!80] (0,0,0) -- (0,0,100) -- (50,0,100) -- (50,0,0) -- cycle;


\filldraw[color=blue!60] (50,0,0) -- (50,0,100) -- (100,50,100) -- (100,50,0) -- cycle;


\filldraw[color=blue!40] (100,50,0) -- (100,50,100) -- (100,100,100) -- (100,100,0) -- cycle;


\filldraw[color=blue!20] (0,0,100) -- (0,50,100) -- (50,100,100) -- (100,100,100) -- (100,50,100) -- (50,0,100) -- cycle;

\end{axis}

\end{tikzpicture}

==> tikz/Old/old_low_influence_3D.tex <==
\begin{tikzpicture}


\begin{axis}[width=6cm, height=6cm,stack plots=y,thick,smooth,no markers,xmin=0,xmax=1,ymin=0,ymax=1,zmin=0,zmax=1,xlabel={$x$},
  ylabel={$y$},zlabel={$z$},xtick={0,0.5,1},ytick={0.5,1},ztick={0.5,1},view={60}{30}]
  

\draw[color=black] (0,0,10) -- (50,0,10);
\draw[color=black] (0,0,20) -- (50,0,20);
\draw[color=black] (0,0,30) -- (50,0,30);
\draw[color=black] (0,0,40) -- (50,0,40);
\draw[color=black] (0,0,50) -- (50,0,50);
\draw[color=black] (0,0,60) -- (50,0,60);
\draw[color=black] (0,0,70) -- (50,0,70);
\draw[color=black] (0,0,80) -- (50,0,80);
\draw[color=black] (0,0,90) -- (50,0,90);
\draw[color=black] (0,0,100) -- (50,0,100);

\draw[color=black] (50,0,10) -- (0,50,10);
\draw[color=black] (50,0,20) -- (0,50,20);
\draw[color=black] (50,0,30) -- (0,50,30);
\draw[color=black] (50,0,40) -- (0,50,40);
\draw[color=black] (50,0,50) -- (0,50,50);
\draw[color=black] (50,0,60) -- (0,50,60);
\draw[color=black] (50,0,70) -- (0,50,70);
\draw[color=black] (50,0,80) -- (0,50,80);
\draw[color=black] (50,0,90) -- (0,50,90);
\draw[color=black] (50,0,100) -- (0,50,100);

\draw[color=black] (10,0,0) -- (10,0,100);
\draw[color=black] (20,0,0) -- (20,0,100);
\draw[color=black] (30,0,0) -- (30,0,100);
\draw[color=black] (40,0,0) -- (40,0,100);
\draw[color=black] (50,0,0) -- (50,0,100);


\draw[color=black] (0,10,100)  -- (40,10,100);
\draw[color=black] (0,20,100)  -- (30,20,100);
\draw[color=black] (0,30,100)  -- (20,30,100);
\draw[color=black] (0,40,100)  -- (10,40,100);

\draw[color=black] (40,10,100) -- (40,10,0);
\draw[color=black] (30,20,100) -- (30,20,0);
\draw[color=black] (20,30,100) -- (20,30,0);
\draw[color=black] (10,40,100) -- (10,40,0);


\draw[color=black] (10,0,100) -- (10,40,100);
\draw[color=black] (20,0,100) -- (20,30,100);
\draw[color=black] (30,0,100) -- (30,20,100);
\draw[color=black] (40,0,100) -- (40,10,100);

\draw[color=black] (50,0,100) -- (0,50,100);
\draw[color=black] (0,50,100) -- (0,50,100);
\draw[color=black] (0,50,100) -- (0,50,0);
\draw[color=black] (0,50,0) -- (50,0,0);





\filldraw[color=blue!80] (0,0,0) -- (0,0,100) -- (50,0,100) -- (50,0,0) -- cycle;


\filldraw[color=blue!40] (50,0,0) -- (50,0,100) -- (0,50,100) -- (0,50,0) -- cycle;


\filldraw[color=blue!20] (0,0,100) -- (0,50,100) -- (50,0,100) -- cycle;

\end{axis}

\end{tikzpicture}

==> tikz/Old/old_tilted_low_influence_3D.tex <==
\begin{tikzpicture}

\begin{axis}[width=6cm, height=6cm,stack plots=y,thick,smooth,no markers,xmin=0,xmax=1,ymin=0,ymax=1,zmin=0,zmax=1,xlabel={$x$},
  ylabel={$y$},zlabel={$z$},xtick={0,0.5,1},ytick={0.5,1},ztick={0.5,1},view={70}{30}]
  

\draw[color=black] (0,0,10) -- (50,0,10);
\draw[color=black] (0,0,20) -- (50,0,20);
\draw[color=black] (0,0,30) -- (50,0,30);
\draw[color=black] (0,0,40) -- (50,0,40);
\draw[color=black] (0,0,50) -- (50,0,50);
\draw[color=black] (0,0,60) -- (50,0,60);
\draw[color=black] (0,0,70) -- (50,0,70);
\draw[color=black] (0,0,80) -- (50,0,80);
\draw[color=black] (0,0,90) -- (50,0,90);
\draw[color=black] (0,0,100) -- (50,0,100);

\draw[color=black] (50,0,10) -- (0,50,10);
\draw[color=black] (50,0,20) -- (0,50,20);
\draw[color=black] (50,0,30) -- (0,50,30);
\draw[color=black] (50,0,40) -- (0,50,40);
\draw[color=black] (50,0,50) -- (0,50,50);
\draw[color=black] (50,0,60) -- (0,50,60);
\draw[color=black] (50,0,70) -- (0,50,70);
\draw[color=black] (50,0,80) -- (0,50,80);
\draw[color=black] (50,0,90) -- (0,50,90);
\draw[color=black] (50,0,100) -- (0,50,100);

\draw[color=black] (10,0,0) -- (10,0,100);
\draw[color=black] (20,0,0) -- (20,0,100);
\draw[color=black] (30,0,0) -- (30,0,100);
\draw[color=black] (40,0,0) -- (40,0,100);
\draw[color=black] (50,0,0) -- (50,0,100);


\draw[color=black] (0,10,100)  -- (40,10,100);
\draw[color=black] (0,20,100)  -- (30,20,100);
\draw[color=black] (0,30,100)  -- (20,30,100);
\draw[color=black] (0,40,100)  -- (10,40,100);

\draw[color=black] (40,10,100) -- (40,10,0);
\draw[color=black] (30,20,100) -- (30,20,0);
\draw[color=black] (20,30,100) -- (20,30,0);
\draw[color=black] (10,40,100) -- (10,40,0);


\draw[color=black] (10,0,100) -- (10,40,100);
\draw[color=black] (20,0,100) -- (20,30,100);
\draw[color=black] (30,0,100) -- (30,20,100);
\draw[color=black] (40,0,100) -- (40,10,100);

\draw[color=black] (50,0,100) -- (0,50,100);
\draw[color=black] (0,50,100) -- (0,50,100);
\draw[color=black] (0,50,100) -- (0,50,0);
\draw[color=black] (0,50,0) -- (50,0,0);





\filldraw[color=blue!80] (0,0,0) -- (0,0,100) -- (50,0,100) -- (50,0,0) -- cycle;


\filldraw[color=blue!40] (50,0,0) -- (50,0,100) -- (0,50,100) -- (0,50,0) -- cycle;


\filldraw[color=blue!20] (0,0,100) -- (0,50,100) -- (50,0,100) -- cycle;

\end{axis}

\end{tikzpicture}

==> tikz/indep_utility_vs_influence.tex <==
\begin{tikzpicture}
\begin{axis}[width=6cm, height=6cm,
stack plots=y,thick,smooth,no markers,xmin=0,xmax=1,ymin=0,ymax=1,xlabel={$\iota$},
  ylabel={$U(\mathcal{M})$},axis on top,xtick={0,0.5,1},ytick={0,0.5,1},ylabel near ticks,xlabel near ticks,samples=2000]

\addplot[blue!80, ultra thick] ({\x},{(2+sqrt(4-8*(1-\x)))/4});

\end{axis}
\end{tikzpicture}

==> tikz/joint_utility_vs_influence.tex <==
\begin{tikzpicture}
\begin{axis}[width=6cm, height=6cm,
stack plots=y,thick,smooth,no markers,xmin=0,xmax=1,ymin=0,ymax=1,xlabel={Influence},
  ylabel={Utility},axis on top,xtick={0,0.5,1},ytick={0,0.5,1},ylabel near ticks,xlabel near ticks,samples=4]

\addplot[blue!80, ultra thick] (x,1/2+x/2);

\end{axis}
\end{tikzpicture}
